LLMExplainer: Large Language Model based Bayesian Inference for Graph Explanation Generation

Recent studies seek to provide Graph Neural Network (GNN) interpretability via multiple unsupervised learning models. Due to the scarcity of datasets, current methods easily suffer from learning bias. To solve this problem, we embed a Large Language Model (LLM) as knowledge into the GNN explanation network to avoid the learning bias problem. We inject LLM as a Bayesian Inference (BI) module to mitigate learning bias. The efficacy of the BI module has been proven both theoretically and experimentally. We conduct experiments on both synthetic and real-world datasets. The innovation of our work lies in two parts: 1. We provide a novel view of the possibility of an LLM functioning as a Bayesian inference to improve the performance of existing algorithms; 2. We are the first to discuss the learning bias issues in the GNN explanation problem.

==> introduction_0328.tex <==
\section{Introduction}
\label{sec:intro}
%\begin{itemize}
%\item Para. 1: Introduction to Graph and GNN explanations

Interpreting the decisions made by Graph Neural Networks (GNNs)~\citep{scarselli09gnnmodel} is crucial for understanding their underlying mechanisms and ensuring their reliability in various applications. With the rapidly increasing demand on graph tasks including social networks~\citep{fan19social, min21social}, molecular structures~\citep{chereda2019utilizing, mansimov19deepggnn}, traffic flows~\citep{wang20traffic, Li_Zhu_2021_traffic, wu19graphwave, ijcai2018p0505}, and knowledge graphs~\citep{sorokin-gurevych-2018-modeling-knowledgegraph},
GNNs, with their message-passing mechanisms, propagate and fuse messages from neighboring nodes on the graph, achieving state-of-the-art performance in tasks including node classification, graph classification, graph regression, and link prediction. 
% Recent efforts have focused on enhancing GNN interpretability through the use of multiple unsupervised learning models. 
% However, a common challenge faced by these methods is the risk of over-fitting due to limited datasets.
Improving the interpretability of GNNs and understanding how GNNs make predictions is crucial. First, it can increase the models' transparency and user confidence when using GNNs in high-stakes applications~\citep{yuan2022explainability,longa2022explaining}. Second, it could help people gain more insights from pre-trained models in sensitive fields such as healthcare and drug discovery~\citep{zhang2022trustworthy,wu2022survey,li2022survey}, which require a lot of expert knowledge traditionally without explanations. Therefore, exploring the interpretability of GNNs is essential. 

% \jy{***Re-write introduction, intuition becomes over-fitting by bayesian inference, then introduce LLM as the bayesian knowledge}
% A common solution to improve GNN models' transparency is applying post-hoc instance-level explainability methods. These methods identify key substructures in input graphs to explain predictions made by trained GNN models, making it easier for humans to understand the models' inner workings. Examples of such methods include GNNExplainer~\citep{ying2019gnnexplainer}, which determines the importance of nodes and edges through perturbation, and PGExplainer\citep{luo2020parameterized}, which trains a graph generator to incorporate global information. Recent studies in the field~\citep{fang2023on, NEURIPS2021_be26abe7} also contribute to the development of these methods. Post-hoc explainability methods can be classified under a label-preserving framework, where the explanation is a substructure of the original graph and preserves the information about the predicted label. On top of the intuitive principle, Graph Information Bottleneck (GIB)~\citep{wu2020graph,miao2022interpretable,yu2020graph} maximizes the mutual information $I(G^{*}, Y)$ between the target label $Y$ and the explanation $G^{*}$ while constraining the size of the explanation as the mutual information between the original graph $G$ and the explanation $G^{*}$.
% \jy{rephrase the introduction to be different to the previous paper...}

% Based on the nature of the GNN explainer, it tends to overfit significantly.
% \jy{ask jx to change the first sentence} 

% \jx{para2: introduce the challenge}
\begin{wrapfigure}[15]{r}{0.4\textwidth}
\vspace{-0.3cm}
\begin{center}
     \includegraphics[width=0.4\textwidth]{figures/intuition.png}
    \caption{Intuitive visualization of learning bias.}
    \label{fig: intui}
\end{center}
\end{wrapfigure}
Plenty of recent efforts~\cite{ying2019gnnexplainer, luo2020parameterized, zhang2023mixupexplainer} have focused on enhancing GNN interpretability through multiple learning objectives, especially graph information bottleneck (GIB)~\cite{wu2020graph}.
However, the graph datasets with ground truth explanations are rare because they need much human expert effort to label and some of them have unreasonable mechanisms. Thus, these methods faced a serious challenge: the risk of learning bias due to the scarcity and insufficiency of datasets and the mismatch between the learning objective and performance metric. We intuitively show this learning bias phenomenon in Fig.~(\ref{fig: intui}) and experimentally demonstrate it in Fig.~(\ref{fig: RQ2}).
% \hua{The last sentence seems coming out of nowhere. Either this is a commonly acknowledged problem, or we should support with our results.}
As shown in Fig.~(\ref{fig: intui}), due to the scarcity of the explanation dataset and ground truth and the design of the objective function, the learning bias problem is hard to avoid in the explaining procedure. With the increasing training steps, the explainer is trained to optimize the mutual information $I(G^*, Y)$ between sub-graph $G^*$ and label $Y$. In the left part, the model is under-fitting, where the $I(G^*, Y)$ and the actual performance $\text{AUC}(G^*)$ is increasing. However, in the right part, after the optimized point, while the explainer keeps trying to optimize the $I(G^*, Y)$ as the objective function, it's suffering the learning bias. The $I(G^*, Y)$ is increased with a biased out-of-distribution sub-graph $G^*$, where the AUC performance of $G^*$ drops.
Current models often overlook this issue and instead terminate the learning process at an earlier stage to avoid learning bias. However, in real-world applications, this solution may lead to under-fitting problems, because we don't have a validation dataset with ground truth to determine the early stop point. 
% The main challenges in addressing this problem are twofold: First, since the dataset is relatively small, finding the optimal epoch to end the unsupervised learning process is one potential solution. However, the primary challenge lies in determining when to terminate the process. 

In this paper, we proposed incorporating knowledge through Bayesian Inference, with the knowledge being sourced from a Large Language Model (LLM). By leveraging an LLM as an external expert, we can effectively assess the status of the learning process, make informed decisions, and avoid of learning bias. This approach subsequently helps mitigate the learning bias problem while ensuring that the model achieves a satisfactory level of performance.
% \jy{Check the 5-th line. Did we do that?} \jx{Yes, we use PGExplainer as backbone in experiments}
To enhance the efficiency of Graph Neural Network (GNN) explanation, we introduce \ours, a framework designed to expedite the GNN explanation process embedded with the Bayesian Inference Process. We adopt the Large Language Model (LLM) as a grader to provide prior knowledge to avoid learning bias. \ours can be easily integrated into various types of GNN explanation models, including instance-level explanation models\citep{rgexp, ying2019gnnexplainer, luo2020parameterized, subgraphx, spinelli2022meta, wang2021causal} and model-level explanation models\citep{ying2019gnnexplainer, subgraphx, rgexp}. 
% \jy{add both types of experiments?} \jx{We don't have to, just mention this.}
This framework comprises two key components: a feedback module and the LLM grader. We employ the LLM as a grader to evaluate the scores of each explanation candidate, subsequently incorporating these scores into the model to facilitate weighted gradient descent with the feedback module. With the integration of \ours, existing GNN explanation models demonstrate accelerated convergence and more robustness to learning bias. We theoretically establish that the presence of \ours ensures that the lower bound remains no less than that achieved without its inclusion.



Our main contributions are: % \jy{waiting to change}
\begin{itemize}
    \item We propose a new and general framework, \ours, which solves the problem of learning bias in the graph explanation process by embedding the Large Language Model into the graph explainer with a Bayesian inference process and improving the explanation accuracy. 
    \item We theoretically prove the effectiveness of the proposed algorithm and show that the lower bound of \ours is no less than the original bound of baselines. Our proposed method achieved the best performance through five datasets compared to the baselines.
    \item We are the first to discuss this learning bias problem in the domain of graph explanation and provide the potential of the Large Language Model as a Bayesian inference module to benefit the current works.
\end{itemize}


% \jy{To Be Done By JX: 1. Related work, combine 2.1 and 2.2 2. Experimental 3. Preliminary\\ TBD by JY: 1. Related work BI and LLM 2. Check reference(done) 3. Overall rephrase,etc}
